Controlling Congestion via In-Network Content Adaptation

Realizing that it is inherently difficult to precisely match the sending rates at the endhost with the available capacity on dynamic cellular links, we build a system, Octopus, that sends real-time data streams over cellular networks using an imprecise controller (that errs on the side of over-estimating network capacity), and then drops appropriate packets in the cellular network buffers to match the actual capacity. We design parameterized primitives for implementing the packet dropping logic, that the applications at the endhost can configure differently to express different content adaptation policies. Octopus transport encodes the app-specified parameters in packet header fields, which the routers parse to execute the desired dropping behavior. Our evaluation shows how real-time applications involving standard and volumetric videos can be designed to exploit Octopus, and achieve 1.5-50 times better performance than state-of-the-art schemes.

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Data transfers over the Internet typically involve a congestion controller at the endhost that uses feedback from the network to estimate the available capacity, and accordingly adjusts the data sending rate. Such an approach avoids excessive in-network packet drops, and has worked well for most bulk-transfer applications that require their entire content to be reliably delivered (e.g. file transfer and email).
%\fixme{replace legacy with bulk transfer}

A similar approach was adopted for real-time applications (e.g. web conferencing, tele-robotics, AR/VR), which differ from bulk-transfer applications in two key aspects. First, rather than minimizing the overall flow completion time, real-time applications require minimizing the latency of individual \emph{messages} in the stream, where each message may comprise of one or more packets (e.g. ensuring the delivery of the latest frame in a video stream as quickly as possible). Second, such applications do not require all of the generated content to be reliably delivered, and can instead adapt the content (e.g. video frame rate or quality) based on available link capacity in order to meet their latency requirements.
%(e.g. reducing video frame rate or quality under limited bandwidth).  

%\fixme{might need better transition to the next sentence -- perhaps in the form of implications of these aspects on rate controller design.} 
The state-of-the-art transmission schemes for such applications (primarily focusing on real-time video, e.g.~\cite{salsify,awstream, google-gcc, qarc}) use a congestion controller at the endhost that uses network feedback to estimate available capacity, with the application adapting its content (e.g. video quality and frame rate) based on this estimate. Real-time apps require accurate capacity estimation and adaptation.
%Under-utilizing the network link may result in unnecessarily low throughput which may impact an end user's quality of experience or QoE (e.g. the video quality during conferencing).
Under-utilizing the network link may unnecessarily reduce the throughput and content quality, which harms the user's quality of experience (QoE).
On the other hand, high queuing delays due to a more aggressive sending rate would introduce significant lags in message delivery, that also harms QoE.
%, and may have more severe consequences in some applications (e.g. in networked robotics, where slow responses to the latest changes in a robot's environment may result in collisions).

However, last mile cellular link, often the bottleneck for such applications~\cite{sprout, mowie, bursttracker}, exhibits a high degree of capacity fluctuations~\cite{sprout, abc, 5g-study}. 
%This has been well-studied for LTE~\cite{sprout,abc}, and preliminary studies for 5G reveal an even more bursty behaviour due to dynamic obstacles or change in directionality caused by local movements~\cite{5g-study} \fixme{any other studies showing 5G/mmwave's sensitivity to directionality and obstacles?}\fixme{other issues hold for LTE as well. people may not get that 5G has greater directionality issues}. 
Such link capacity variations are difficult to accurately estimate by endhost congestion controllers.~\footnote{We use the term `endhost congestion controller' to refer to any controller that determines the data sending rate at the endhost by estimating link capacity using network feedback (including the ones that use early congestion signals~\cite{ecn, codel} or explicit rate feedback~\cite{rcp, xcp} from the network).}  
%Typical WAN congestion controllers (e.g. Cubic~\cite{cubic} and BBR~\cite{bbr}) are too aggressive and result in high queuing delays. This has led to designing congestion controllers specifically for cellular networks (e.g.~\cite{sprout, verus, abc}). However, as we show in \S\ref{sec:motivation} (and as has been observed earlier~\cite{abc}) these congestion controllers are not perfect either. 
%On the other hand, schemes designed for cellular network (e.g. Sprout~\cite{sprout}) \fixme{The logic is inaccurate here} 
%They may under-utilize the network and still fail to achieve consistently low queuing delays. 
An aggressive congestion controller (e.g. Cubic~\cite{cubic} or BBR~\cite{bbr}) may result in high queuing delays, while a more cautious one may under-utilize the link. In fact, as we show in \S\ref{sec:motivation}, no practical endhost congestion  controller can achieve both high link utilization and consistently low queuing delays under such time-varying capacities. 
%Moreover, our evaluation in \S\ref{sec:casestudies} shows how slow application-level adaptation to the estimated bandwidth further impacts performance.   
%As we show in \S\ref{sec:casestudies}, this combined with sub-optimal application-layer adaptation, degrades application performance. 
%that can receive feedback from the network only after one round-trip time, and end up being either too aggressive (resulting in high queuing delays) or too cautious (resulting in low link utilization) \fixme{revisit -- expand a bit, differentiating default Internet CC from Sprout-like approaches and the Oracle result}. 
%Moreover, our evaluation in \S\ref{sec:casestudies} reveals additional sources of inefficiencies in how applications adapt to the estimated bandwidth, that further impact application performance. \fixme{todo: elaborate}   

\input{motivation-fig}

In this paper, we propose an alternative approach that exploits smarter in-network buffer management to circumvent the above issues, and achieve both high throughput and low latency for real-time applications. The key idea is to allow the endhosts to send data using an aggressive congestion controller (we use BBR), so as to maximize throughput. Then, when the link capacity decreases or when queues start building up at the cellular router, it selectively drops packets using semantic cues encoded in the packet headers. For example, in a sensor stream for a robotics or an AR/VR application, which requires processing the freshest information, the router can drop an older queued up message which loses its value upon the arrival of a newer message. In a layer-encoded video stream for real-time conferencing, the router can drop higher quality layers when bandwidth is limited. Our proposed router logic is app-agnostic, and implements general dropping primitives (parameterized by packet header fields) that a real-time app can instantiate differently at the endhost to support different semantic requirements.

%Note that while we motivate our work in the context of cellular base-stations, it is also applicable for switches elsewhere along the network path, e.g. at the edge of an ISP, 
%(which can be a source of inter-domain congestion~\cite{inter-domain}, with the available per-user bandwidth fluctuating with traffic patterns) 
%and at WiFi access points.  

%The idea of exploiting in-network buffer management techniques to improve performance is certainly not new. Many different scheduling policies have been proposed in the context of both wide-area and datacenter networks~\cite{diffserv,drr,fq,gps,pfabric,pifo}, which primarily focus on the complementary problem of scheduling across different flows (e.g. to achieve fairness or small flow completion time). An intra-flow scheduling scheme (e.g.~\cite{bedewey2019, kadota2019}) would essentially reorder transmissions within a flow, which is ill-suited for real-time applications
%They maintain in-order transmissions within a flow,~\footnote{We discuss a few exceptions~\cite{bedewey2019, kadota2019} in \S\ref{sec:related}.} which in fact is desirable in real-time applications
%. \fixme{cut?}} 
%In fact, maintaining the temporal ordering of messages within a stream is indeed the best choice for real-time applications 
%(there is little value to delivering an older message out-of-order, after a later message in the stream has been delivered). Different from scheduling, the key question we consider is whether a message in a given real-time stream should be transmitted by the router or dropped altogether. 

%In that context, ``intelligent packet discard'' was proposed more than two decades ago as a use-case of active networking~\cite{zegura-an, bhattacharjee1998network}, which specifically looked at video transfers. However, rather than minimizing queuing delay, its goal was to ensure that when the router buffer overflows, certain lower priority video frames are discarded over more useful ones.
%~\footnote{One could argue that the queuing delay can be minimized with such an approach by appropriately tuning the router buffer size. However, buffer size tuning is notoriously difficult for cellular links with time-varying bandwidths~\cite{sprout}. Moreover, the appropriate buffer size would also depend on message sizes which too vary over the duration of the application, and thus cannot be pre-configured.} 
%The discard policy also accounted for frame dependencies, which required programming application-specific logic and state in the routers.
%based on specific video formats. 
%(We discuss this in more details, along with other related work which have similar limitations, in \S\ref{sec:related}.) 
%\fixme{something on priority scheduling}

%It proposed a priority dropping policy for MPEG transfers, that favored dropping certain lower priority video frames when the router buffer became full. The packet drop policy   
%Intelligent packet discard, other forms of MPEG filters,...(i) Look at specific policies for specific video formats, and expect in-network elements to be aware of such policies (to be pre-programmed with application specific logic and maintain application-specific state). Lack general primitives that can support a variety application requirements. (ii) Goal is not to minimize the effects queuing delay. Rather it is to ensure that when buffer is full, certain lower priority frames are discarded over more useful one. Trigger drops only when packet buffer full. One can tune the buffer size, but difficult to do so for cellular network as appropriate size would depend on link bandwidth that fluctuates. Also, for such apps, appropriate buffer size would also depend on message size -- cannot be pre-configured. (iii) Also don't explore the interplay of in-network dropping with transport protocol design -- check.


%Our idea draws some of its inspiration from ``intelligent packet discard'' at network routers, proposed more than two decades ago as a use-case of active networking~\cite{zegura-an}. It was a preliminary proposal that looked at two specific policies in the context of atomic drops for MPEG transfers (namely, dropping an entire frame instead of a packet, and the entire ``group of pictures'' instead of a reference frame). It did not explore different application requirements (e.g. video quality adaptation, data freshness, etc) and how they are specified to the network, nor the interplay of in-network dropping with transport protocol design. \fixme{check} 

%Today, the increased reliance on cellular connectivity to support a growing class of real-time applications (e.g. for smart cities), and the ongoing evolution of cellular infrastructure~\cite{5G-microbook}, provides the right context and a timely opportunity to revisit the idea of smarter in-network dropping policies. However, rather than expecting the routers to be programmed with application-specific logic, we design general primitives (parameterized by packet headers) that an application can instantiate differently at the endhost to support a variety of requirements. Moreover, with our goal of minimizing queuing delays, we use more proactive signals (namely, a new message arrival and the current bandwidth) to trigger packet drops, rather than waiting for the router buffer to fill up.
%to ensure low queuing delays \fixme{fix}.                                                                          


We design a system, \oursys, based on this idea. 
It comprises of: (i) an interface for the applications to specify dropping policies at the granularity of atomic messages using the parameterized dropping primitives, (ii) a message-aware transport protocol that encodes the app-specified policies (parameters) into packet headers, 
% %appropriately handles purposeful in-network drops, 
and performs transport buffer management and congestion control, (iii) router logic for implementing the dropping primitives and parsing the packet header fields to enforce the desired dropping behaviour. 
%\fixme{should we add a line or two stating that applications need to be redesigned to exploit our framework.}
%We use our prototype implementation and emulation testbed (\S\ref{sec:prototype}) to evaluate \oursys. More specifically, via two case-studies,
%We design (\S\ref{sec:design}) and prototype (\S\ref{sec:prototype}) our system, \oursys, based on this approach. 
%\radhika{summarize key aspects of the system. what's cool about our design.}

We use three different case-studies to demonstrate how real-time video streaming apps can be designed to exploit \oursys for different requirements.   
%in two \fixme{hopefully three} different scenarios involving real-time video transmissions. 
Our results show that \oursys can achieve 1.5-18 $\times$ better performance across different scenarios when compared to state-of-the-art approaches~\cite{awstream, salsify}  
%that adapt video quality using an endhost congestion controller
(where better performance is characterized by higher message throughput and lower latency, with similar or higher data quality as per the app requirements).  
%AWStream~\cite{awstream} and \fixme{XX-YY} better performance than Salsify~\cite{salsify} \ammar{Mention of awstream and salsify looks quite abrupt here, we should mention them earlier so reader knows why we are comparing with these.}, 


%This paper shows the promise of our approach, opening several interesting directions for future research (we discuss these in \S\ref{sec:discussion}). 
%\fixme{something forward looking}
%This work does not raise any ethical issues. 

%\alvin{keep it. May shorten some paragraphs}
